Highlights from BESIII experiment

BESIII had collected large data samples on $J/\psi$ and $\psi^\prime$ peaks during the first run in 2009. From 2010 to 2011, about 2.9 fb$^{-1}$ integrated luminosity were obtained on the peak of $\psi(3770)$ for open charm physics. We review recent results on charmonium decays and hadron spectroscopy. The prospects on open charm physics are also discussed.

==> ctextemp_contribution.tex <==
\def\CTeXPreproc{Created by ctex v0.2.12, don't edit!}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% template for hadron2011 contribution
%
% please do not rename this file
%
% to create document run
%
%     pdflatex hadron2011.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{  % do not remove


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% please define your macros here

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% define title, author, and address
% contribution[short title]{title}{author first name}{author last name}{author address}{author email}{collaboration}
% the short title will appear in the page headers and the TOC of the book of proceedings
% the last two arguments may be left empty
\contribution[Highlights from BESIII experiment]  % short title (optional)
{Highlights from BESIII experiment}  % title
{Hai-Bo}{Li}  % first and last name of author
{Institute of High Energy Physics \\
Bejing 100049, China}  % author address
{lihb@ihep.ac.cn}  % author email optional
{on behalf of the BESIII Collaboration}  % collaboration (optional)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% abstract
\abstract{%
BESIII had collected large data samples on $J/\psi$ and
$\psi^\prime$ peaks during the first run in 2009. From 2010 to 2011,
about 2.9 fb$^{-1}$ integrated luminosity were obtained on the peak
of $\psi(3770)$ for open charm physics. We review recent results on
charmonium decays and hadron spectroscopy. The prospects on open
charm physics are also discussed. }
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% main text
% for short contributions sections are optional
\section{Introduction}

The newly built BEPCII/BESIII is an upgrade to the previous
BEPC/BES~\cite{besiii}. The BEPCII is a double ring collider with a
design luminosity of $1\times 10^{33}$cm$^{-2}$s$^{-1}$ at a
center-of-mass energy of 3.78 GeV, which luminosity is one order of
higher than that at CESR-c. It is operating between 2.0 and 4.6 GeV
in the center of mass. The BESIII experiment is used to study the
charm and $\tau$ physics. It is foreseen to collect on the order of
10 billion $J/\psi$ events or 3 billion $\psi(2S)$ events per year
according to the designed luminosity.  About 32 million
$D\overline{D}$ pairs and $2.0$ million $D_S \overline{D}_S$ at
threshold will be collected per year~\cite{besiii}.  In last run,
the peak luminosity of BEPCII has reached $6.4 \times
10^{32}$cm$^{-2}$s$^{-1}$.

The BESIII detector~\cite{besiii}
%as shown in
%Fig.~\ref{fig1:besiii},
consists of the following main components:
1) a main draft chamber (MDC) equipped with about 6500 signal wires
and 23000 field wires arranged as small cells with 43 layers. The
designed single wire resolution is 130 $\mu m$ and the momentum
resolution 0.5\% at 1 GeV; 2) an electromagnetic calorimeter(EMC)
made of 6240 CsI(Tl) crystals. The designed energy resolution is
2.5\%@1.0 GeV and position resolution 6mm@1.0 GeV; 3) a particle
identification system using Time-Of-Flight counters made of 2.4 m
long plastic scintillators. The designed resolution is 80 ps for two
layers, corresponding to a K/$\pi$ separation (2$\sigma$ level) up
to 0.8 GeV; 4)a superconducting magnet with a field of 1 tesla; 5) a
muon chamber system made of Resistive Plate Chambers(RPC).
%\begin{figure}[htb]
%  \begin{center}
%    % please do not add file name extension this makes switching between latex and pdflatex easier
%    \includegraphics[width=0.6\textwidth]{pdf-plot/bes_view}
%   \caption{A schematic view of the BESIII detector.}
%    \label{fig1:besiii}
%  \end{center}
%\end{figure}

In 2009, the BESIII had collected about 225 M and 106M data set on
the J/$\psi$ and $\psi^\prime$ peaks, respectively. About 2.9
fb$^{-1}$ integrated luminosity on the $\psi(3770)$ peak had been
accumulated for open charm physics, and the data size is about 3.5
times of that at CLEO-c. The results in this paper is based above
data set.

\section{Highlights from BESIII}

The BESIII collaboration has published so-far a variety of papers
with many new results in the field of light hadron and charmonium
spectroscopy, as well as charmonium
decays~\cite{hc_paper,gP_paper,PP_paper,ppbar_paper,X1835_paper,matrix_paper,4pi_paper,
mixing_paper,gV_paper,vv_paper}. A number of new hadronic states
were discovered or confirmed, and various decay properties were
measured for the first time. In addition, many data analyses are in
an advanced stage and will lead to a rich set of new publications in
the near future. Here, we show recent highlights from the BESIII,
thereby, illustrating the potential of the BESIII experiment. In
this paper, for the reported experimental results, the first error
and second error will be statistical and systematic, respectively,
if they are not specified.

\subsection{$\eta_c(1S)$ resonance via $\psi^\prime \rightarrow \gamma \eta_c$ decay}

Precise measurement of M1 transition of $\psi^\prime$ is important
for us to understand the QCD in the relativistic and nonperturbative
regimes.  The $\psi^\prime \rightarrow \gamma \eta_c$ transition is
also a source of information on the $\eta_c$ mass and width. There
is currently a 3.3 $\sigma$ inconsistency in previous $\eta_c$ mass
measurements from J$/\psi$ and $\psi^\prime\rightarrow \gamma
\eta_c$ (averaging $2977.3 \pm 1.3$ MeV/$c^2$) compared to $\gamma
\gamma$ or $p\bar{p}$ production (averaging 2982.6 $\pm$1.0
MeV/$c^2$)\cite{ref:hc-hyper}. The width measurements also spread
from 15 to 30 MeV, it is around 10 MeV in the earlier days of
experiments using J/$\psi$ radiative transition~\cite{mark3,bes1},
while the recent experiments, including photon-photon fusion and B
decays, gave higher mass and much wider
width~\cite{cleo-c,babar,belle1,belle2}. The most recent study by
the CLEO-c experiment~\cite{cleo-c-new}, using both $\psi^\prime$
and J/$\psi \rightarrow \gamma \eta_c$ decays, and pointed out there
was a distortion of the $\eta_c$ line shape. CLEO-c attributed the
$\eta_c$ line-shape distortion to the energy-dependence of the M1
transition matrix element. In the $J/\psi \rightarrow \gamma \eta_c$
from CLEO-c, the distorted $\eta_c$ lineshape can be described by
the relativistic Breit-Wigner (BW) distribution modified by a factor
of E$^3_{\gamma}$ together with a dumping factor to suppress the
tail on the higher photon energies. KEDR Collaboration did the same
thing but tried different dumping factor~\cite{kedr}.

Based on the data sample of 106 M $\psi^\prime$ events collected
with BESIII detector,  the $\eta_c$ mass and width are measured from
the radiative transition $\psi^\prime \rightarrow \gamma \eta_c$.
The $\eta_c$ candidates are reconstructed from six exclusive decay
modes: $K_s K\pi$, $K^+K^-\pi^0$, $\eta \pi^+\pi^-$, $K_s
K^+\pi^-\pi^+\pi^-$, $K^+K^-\pi^+\pi^-\pi^0$, and 3$(\pi^+\pi^-)$,
where $K_s$ is reconstructed in  $\pi^+\pi^-$ mode, $\eta$ and
$\pi^0$ from $\gamma \gamma$ final states. For a hindered M1
transition the matrix element acquires terms proportional to
$E^2_{\gamma}$, which, when combined with the usual $E^3_{\gamma}$
term for the allowed transitions, lead to contributions in the
radiative width proportional to $E^7_{\gamma}$. Thus, the $\eta_c$
lineshape is described by a BW modified by $E_{\gamma}^7$ convoluted
with a resolution function. It is important to point out that the
interference between $\eta_c$ and non-resonance in the signal region
is also considered. The statistical significance of the interference
is 15 $\sigma$. This affects the $\eta_c$ resonant parameters
significantly. Assuming an universal relative phase between the two
amplitudes, we obtain $\eta_c$ mass and width, $M = 2984.2 \pm 0.6
\pm 0.5$ MeV/$c^2$ and $\Gamma = 31.4 \pm 1.2 \pm 0.6$ MeV,
respectively, as well as the relative phase $\phi = 2.41 \pm
0.06\pm0.04$ rad. Figure~\ref{fig:eta-c-shape} shows the fit results
in the six $\eta_c$ decay modes. With precise measurement of the
$\eta_c$ mass, one can obtain the hyperfine splitting, $\Delta
M_{hf}(1S)_{c\bar{c}} \equiv = M(J/\psi) - M(\eta_c) = 112.5 \pm
0.8$ MeV, which agrees with the quark model prediction~\cite{kseth},
and will be helpful for understanding the spin-dependent
intera

==> ctextemp_contributionmacros.tex <==
\def\CTeXPreproc{Created by ctex v0.2.12, don't edit!}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros for single contribution


% contribution[short title]{title}{author first name}{author last name}{author address}{author email}{collaboration}
\newcommand{\contribution}[7][]{%
  \clearpage
  \thispagestyle{plain}
  \ifthenelse{\equal{#1}{}}
  {\hypersetup{pdftitle={#2}}}
  {\hypersetup{pdftitle={#1}}}
  \hypersetup{pdfauthor={{#3} {#4}}}
  {\centering\normalfont\LARGE\bfseries\sffamily #2 \par\nobreak}
  \lhead{}
  \chead{%
    \textit{\footnotesize XIV International Conference on Hadron Spectroscopy
      (\weblink[\textit{hadron2011}]{http://www.hadron2011.de}), 13-17 June 2011, Munich, Germany}%
  }
  \rhead{}
  \bigskip
  \begin{center}
    {#3} {#4}\ifthenelse{\equal{#6}{}}{}{\footnote{\weblink[#6]{mailto:#6}}}
    \ifthenelse{\equal{#7}{}}{}{#7} \\
    \textit{#5}
  \end{center}
  \bigskip
}


\renewcommand{\abstract}[1]{%
  \begin{center}
    \begin{minipage}{0.85\textwidth}
      \begin{footnotesize}
        #1
      \end{footnotesize}
    \end{minipage}
  \end{center}
  \bigskip
}


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> ctextemp_econfmacros.tex <==
\def\CTeXPreproc{Created by ctex v0.2.12, don't edit!}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% some macros for econf proceedings articles


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% layout macros

% \weblink}[shown text]{URL}
\newcommand{\weblink}[2][]{%
    \ifthenelse{\equal{#1}{}}%
    {\textnormal{\url{#2}}}%
    {\textnormal{\href{#2}{#1}}}%
}

\newcommand{\acknowledgements}[1]{%
  \bigskip\bigskip
  \textsf{\textbf{\Large Acknowledgements}} \\[2ex]
  {#1}
  \bigskip
}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% basic formatting macros

% single-line equations
\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

% multiple-line equations  (use \CR as the carriage return):
\def\beqa{\begin{eqnarray}}
\def\eeqa#1{\label{#1}\end{eqnarray}}
\def\eeqan{\end{eqnarray}}
\def\CR{\nonumber \\ }

% reference to an equation number:
\def\leqn#1{(\ref{#1})}

% sizing and bars
\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}
\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% text-mode macros
\def\etal{{\it et al.}}
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% expectation values
\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% caligraphic letters (for matrix elements, luminosity, etc.)
\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% matrix operations and fractions
\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% high-energy physics terminology
\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_h}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\msb{{\bar{\ssstyle M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% supersymmetry
\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

